Probabilistic Regression with Huber Distributions

In this paper we describe a probabilistic method for estimating the position of an object along with its covariance matrix using neural networks. Our method is designed to be robust to outliers, have bounded gradients with respect to the network outputs, among other desirable properties. To achieve this we introduce a novel probability distribution inspired by the Huber loss. We also introduce a new way to parameterize positive definite matrices to ensure invariance to the choice of orientation for the coordinate system we regress over. We evaluate our method on popular body pose and facial landmark datasets and get performance on par or exceeding the performance of non-heatmap methods. Our code is available at github.com/Davmo049/Public_prob_regression_with_huber_distributions

==> figsAndTables/Loss_WFLW_ablation.tex <==
\begin{table}[]
  \centering
      \caption{Wflw ablation text}
    \begin{tabular}{lcc}
    \toprule
    Loss type & NME ($\downarrow$) & NLL ($\downarrow$)\\
    \midrule
        Prob. Huber($\nu$) & 4.91 $\pm$ 0.04 & -355.8 $\pm$ 0.79 \\
       Prob. Huber($\mu$) & 5.00 $\pm$ 0.07 & -349.7 $\pm$ 2.10 \\
         L2 & 5.16 $\pm$ 0.03 & - \\
         Squared L2 & 
         6.04 $\pm$ 0.10 & - \\
         Huber & 5.52 $\pm$ 0.02 & - \\
    \bottomrule
    \end{tabular}
    \label{tab:WFLW_loss_ ablation}
\end{table}

==> figsAndTables/Mpii_ablation.tex <==
\begin{table}[htbp]
    \centering
    \caption{MPII ablation text}
    \begin{tabular}{c c c c}
         \bottomrule
         Loss & Epochs & PCKh@0.5 ($\uparrow$) & Fusion type\\
         \bottomrule
         Prob. Huber($\nu$) & 200 & 85.4 $\pm$ 0.2 & probabilstic\\
         Prob. Huber($\nu$) & 50  & 85.0 $\pm$ 0.1 & probabilstic \\
         Prob. Huber($\nu$) & 50  & 84.8 $\pm$ 0.1 & mean \\ 
         Prob. Huber($\mu$) & 50  & 85.3 $\pm$ 0.2 & probabilstic \\
         Squared L2         & 50  & 77.0 $\pm$ 0.1 & mean\\
         L2                 & 50  & 82.8 $\pm$ 0.1 & mean \\
         Huber              & 50  & 81.9 $\pm$ 0.1 & mean\\
         \bottomrule
    \end{tabular}
    \label{tab:mpii_ablation_table}
\end{table}


==> figsAndTables/Wflw_Ablation.tex <==
\begin{table}[htbp]
  \centering
      \caption{Loss ablation for WFLW.}
      \bobcaptionspace
    \begin{tabular}{lcllcccc}
      \toprule
      \multicolumn{2}{c}{\textbf{Architecture}} &
      \multicolumn{4}{c}{\textbf{Training \& Test Set-up}} & \multicolumn{2}{c}{\textbf{Results}}\\
      \cmidrule(r){1-2} \cmidrule(r){3-6} \cmidrule(r){7-8}
      Network & Avg. pool & Loss & Pretrain & TTA & Epochs & NME ($\downarrow$) & NLL ($\downarrow$) \\
      \midrule
         ResNet101 & \xmark & Our & 300W-LP\cite{zhu2016face} & \checkmark & 200 & 4.58 $\pm$ 0.02 & - \\
         ResNet101 & \xmark & Our & ImageNet & \checkmark & 200 & 4.62 $\pm$ 0.04 & - \\
         ResNet101 & \xmark & Our & 300W-LP\cite{zhu2016face} & \xmark & 200 & 4.70 $\pm$ 0.03 & -344.6 $\pm$ 1.60 \\
         ResNet101 & \xmark & Our & ImageNet & \xmark & 200 & 4.76 $\pm$   0.06 & -355.4 $\pm$  3.30 \\
         ResNet101 & \xmark & Our & ImageNet & \xmark & 50 & 4.91 $\pm$ 0.04 & -355.8 $\pm$ 0.79 \\
         ResNet50  & \xmark & Our & ImageNet & \xmark & 50 & 4.89 $\pm$ 0.02 & -357.2 $\pm$ 0.47\\
         ResNet18  & \xmark & Our & ImageNet & \xmark & 50 & 5.01 $\pm$ 0.02 & -351.0 $\pm$ 0.75\\
         ResNet101 & \checkmark & Our & ImageNet  & \xmark & 50 & 5.25 $\pm$ 0.02 & -336.5 $\pm$ 0.40  \\
         ResNet101 & \xmark & Our & None & \xmark & 50 & 5.31 $\pm$ 0.04 & -342.2 $\pm$ 1.20 \\
         ResNet101 & \xmark & Our ($\mu$ param) & ImageNet & \xmark & 50 & 5.00 $\pm$ 0.07 & -349.7 $\pm$ 2.10 \\
         ResNet101 & \xmark & L2 & ImageNet & \xmark & 50 & 5.16 $\pm$ 0.03 & - \\
         ResNet101 & \xmark & Squared L2 & ImageNet & \xmark & 50 & 6.04 $\pm$ 0.10 & - \\
         ResNet101 & \xmark & Huber & ImageNet & \xmark & 50 & 5.52 $\pm$ 0.02 & - \\
         \bottomrule
    \end{tabular}
    \label{tab:WFLW_ablation}
\end{table}


==> figsAndTables/arch.tex <==
\begin{figure}[htpb]
\centering
\def\pwid{\textwidth}
\includegraphics[width=\pwid, trim=0 710 250 0, clip]{images/netarch}
\bobcaptionspace
\caption{Schematic of network architecture for our method}
\label{fig:network_arch}
\end{figure}

==> figsAndTables/mpii_wflw_loss_ablation.tex <==
\begin{table}
  \caption{Results of loss ablation experiments. For each experiment a ResNet101, pre-trained with ImageNet, was trained for 50 epochs with one of the five losses below.  For the MPII dataset we apply test time augmentation with mean fusion and no test-time augmentations for the WFLW dataset.}
  \bobcaptionspace
  \hspace{0.05\textwidth}
  \begin{subtable}[t]{0.4\textwidth}
    \subcaption{\normalsize WFLW}
    \raggedright
    \begin{tabular}{lc}
      \toprule
      %% & \multicolumn{2}{c}{\textbf{Results}}\\
      %% \cmidrule(r){2-3}
      Loss & NME ($\downarrow$) \\
      \midrule
      Prob. Huber($\nu$) & \textbf{4.91} $\pm$ .04 \\              
      Prob. Huber($\mu$) & 5.00 $\pm$ .07 \\
      Huber & 5.52 $\pm$ .02 \\                            
      $L_2$ & 5.16 $\pm$ .03 \\
      Squared $L_2$ & 6.04 $\pm$ .10 \\
      \bottomrule
    \end{tabular}
  \end{subtable}%
  \hfill
  \begin{subtable}[t]{0.4\textwidth}        
    \raggedleft
    \caption{\normalsize MPII}
    \begin{tabular}{l r c c}
         \toprule
         Loss & PCKh@0.5 ($\uparrow$)\\
         \midrule
         Prob. Huber($\nu$) & 84.8 $\pm$ 0.1\\
         Prob. Huber($\mu$) & \textbf{85.3} $\pm$ 0.2\\
         Huber              & 81.9 $\pm$ 0.1\\
         $L_2$              & 82.8 $\pm$ 0.1\\         
         Squared $L_2$      & 77.0 $\pm$ 0.1\\
         %% Prob. Huber($\nu$) & 200 & 85.4 $\pm$ 0.2 & probabilstic\\
         %% Prob. Huber($\nu$) & 50  & 85.0 $\pm$ 0.1 & probabilstic \\
         %% Prob. Huber($\nu$) & 50  & 84.8 $\pm$ 0.1 & mean \\ 
         %% Prob. Huber($\mu$) & 50  & 85.3 $\pm$ 0.2 & probabilstic \\
         %% Squared L2         & 50  & 77.0 $\pm$ 0.1 & mean\\
         %% L2                 & 50  & 82.8 $\pm$ 0.1 & mean \\
         %% Huber              & 50  & 81.9 $\pm$ 0.1 & mean\\
         \bottomrule         
    \end{tabular}
  \end{subtable}
  \hspace{0.05\textwidth}
  \label{tab:mpii_wflw_loss_ablation}
\end{table}

==> figsAndTables/mpii_wflw_tta_ablations.tex <==
\begin{table}
  \caption{Results of TTA fusion ablation experiments}
  \subcaptionspace
    \begin{subtable}[t]{0.4\textwidth}
      \subcaption{\normalsize WFLW}
      \raggedright
      \begin{tabular}{lcrr}
        \toprule
        %% Loss & NME ($\downarrow$) & NLL ($\downarrow$) \\
        %% \midrule
        TTA fusion & NME ($\downarrow$) & NLL ($\downarrow$) \\
        \midrule
        MLE & 4.58 $\pm$ 0.02 & n/a \\
        Mean & 4.59 $\pm$ 0.02 & n/a \\
        %ImageNet & MLE & 4.62 & n/a \\
        none & 4.70 $\pm$ 0.03 & -344.6 $\pm$ 1.6\\
        %ImageNet & none & 4.76 & -355.4\\        
        \bottomrule
      \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.4\textwidth}
    \raggedleft
      \caption{\normalsize MPII}
      \begin{tabular}{lcr}
        \toprule
        TTA fusion & PCKh@0.5 ($\uparrow$)\\
        \midrule
        MLE &  85.4 $\pm$ 0.2\\
        Mean &  85.3 $\pm$ 0.2\\
%        Prob. Huber($\nu$)* & MLE  & 85.4 $\pm$ 0.2\\
 %       Prob. Huber($\nu$)* & Mean  & 85.3 $\pm$ 0.2\\
%        Prob. Huber($\nu$) & MLE  & 85.0 $\pm$ 0.1\\
%        Prob. Huber($\nu$) & Mean & 84.8 $\pm$ 0.1\\
%        Prob. Huber($\mu$) & MLE  & 85.3 $\pm$ 0.2\\
 %       Prob. Huber($\mu$) & Mean & ??\\        
        %% ResNet101 & 4.91 $\pm$ 0.04 & -355.8 $\pm$ 0.79 \\
        %% ResNet50 & 4.89 $\pm$ 0.02 & -357.2 $\pm$ 0.47\\
        %% ResNet18 & 5.01 $\pm$ 0.02 & -351.0 $\pm$ 0.75\\
        \bottomrule
      \end{tabular}
    \end{subtable}              
    %% \fbox{\begin{subtable}[t]{0.5\textwidth}
    %%   \subcaption{\normalsize MPII - TTA fusion}
    %%   \raggedleft
    %%   \begin{tabular}{@{}lcr@{}}
    %%     \toprule
    %%     Loss & TTA fusion & PCKh@0.5 ($\downarrow$)\\
    %%     \midrule
    %%     Prob. Huber($\nu$)* & MLE  & 85.4 $\pm$ 0.2\\        
    %%     Prob. Huber($\nu$) & MLE  & 85.0 $\pm$ 0.1\\
    %%     Prob. Huber($\nu$) & Mean & 84.8 $\pm$ 0.1\\
    %%     Prob. Huber($\mu$) & MLE  & 85.3 $\pm$ 0.2\\
    %%     Prob. Huber($\mu$) & Mean & ??\\        
    %%     %% ResNet101 & 4.91 $\pm$ 0.04 & -355.8 $\pm$ 0.79 \\
    %%     %% ResNet50 & 4.89 $\pm$ 0.02 & -357.2 $\pm$ 0.47\\
    %%     %% ResNet18 & 5.01 $\pm$ 0.02 & -351.0 $\pm$ 0.75\\
    %%     \bottomrule
    %%   \end{tabular}
    %% \end{subtable}}      
\end{table}
